Fair Grading Algorithms for Randomized Exams

This paper studies grading algorithms for randomized exams. In a randomized exam, each student is asked a small number of random questions from a large question bank. The predominant grading rule is simple averaging, i.e., calculating grades by averaging scores on the questions each student is asked, which is fair ex-ante, over the randomized questions, but not fair ex-post, on the realized questions. The fair grading problem is to estimate the average grade of each student on the full question bank. The maximum-likelihood estimator for the Bradley-Terry-Luce model on the bipartite student-question graph is shown to be consistent with high probability when the number of questions asked to each student is at least the cubed-logarithm of the number of students. In an empirical study on exam data and in simulations, our algorithm based on the maximum-likelihood estimator significantly outperforms simple averaging in prediction accuracy and ex-post fairness even with a small class and exam size.

==> Body/0_outline.tex <==
\section{Outline}

\paragraph{Introduction}
\begin{itemize}
    \item motivation and overview
    \item why do we need a online exam grading system 
    \item what's the current system (simple averaging and why it is not good)
    \item introduction of benchmark
    \item introduction of model
    \item introduction of algorithm
\end{itemize}

\paragraph{Results.}
\begin{itemize}
    \item existence and uniquencess of the MLEs
    \item its uniform consistency under the BTL model
    \item real-world: cross validation (we have a smaller error, our suggestion for how to choose the degree)
    \item numerical: visualize the unfairness of simple averaging; how to choose the question sample size (5*5);
\end{itemize}

\paragraph{Related work.}

...


Old outline:
\begin{itemize}
    \item motivation+simple statements of a result, random drawing-> unfairness, structural->accuracy+fairness
    \item why do we need a online exam grading system
    \item what's the current system (simple averaging) <- setting (T/F questions, random drawing)
    \item why simple averaging is not good (a running example) <- ex-ante unbiased and ex-post unfair
    \item what do we do? (on this running example)
    
    \item what do we do theoretically and empirically?
    \item existence and uniquencess of the MLEs
    \item its uniform consistency under the BTL model
    \item real-world: cross validation (we have a smaller error, our suggestion for how to choose the degree)
    \item numerical: visualize the unfairness of simple averaging; how to choose the question sample size (5*5);
\end{itemize}

\paragraph{Model}
\begin{itemize}
    \item 
    An abstraction of the exam grading problem.
    \begin{itemize}
        \item Assignment graph: a sparse bipartite
        \item Objective: to measure the probability that a student can answer a random question correctly
        \item Grading rule
    \end{itemize}
\end{itemize}

\paragraph{Method}
\begin{itemize}
    \item Our algorithm, given the exam result as an input, outputs a prediction matrix.
\end{itemize}

\paragraph{Theory}
\begin{itemize}
    \item Theorem 1: Given a random bipartite graph with polylog vertex degree, the resulting directed graph is strongly connected w.h.p.
    \item Theorem 2: the MLE of the BT model is consistent with the parameter under the above assignment graph w.h.p.
    \item Corollary: Our algorithm performs well on the Bradley-Terry model
\end{itemize}

\paragraph{Real-world experiments}
\begin{itemize}
    \item Data description.
    \item Cross-validation.
    \item Calibration index \& Classification index.
\end{itemize}

\paragraph{Simulation (How to visualize?)}
\begin{itemize}
    \item Data description.
    \item The expected performance of (our method / averaging) over a fixed random graph.
    \item The expected bias of (our method / averaging) over different random graphs (use bias for aggregation on one graph)
    \item The expected bias of (our method / averaging) over different number of question samples, given a prior distribution on the question difficulty.
\end{itemize}

==> Body/1_introduction.tex <==
\section{Introduction}

A common approach for deterring cheating in online examinations is to
assign students random questions from a large question bank.  This
random assignment of questions with heterogeneous difficulties leads to
different overall difficulties of the exam that each student faces.
Unfortunately, the predominant grading rule -- simple averaging --
averages all question scores equally and results in an unfair grading
of the students. This paper develops a grading algorithm that utilizes
structural information of the exam results to infer student abilities
and question difficulties.  From these abilities and difficulties
fairer and more accurate grades can be estimated.  This grading
algorithm can also be used in the design of short exams that
maintaining a desired level of accuracy.

During the COVID-19 pandemic, learning management systems (LMS) like
Blackboard, Moodle, Canvas by Instructure, and D2L have benefited
worldwide students and teachers, especially in remote learning
\citep{razaSocialIsolationAcceptance2021}. The current exam module in
these systems includes four steps. In the first step, the instructor
provides a large question bank.  In the second step, the system
assigns each student a distinct random subset of the
questions. (Assigning each student a distinct random subset of the
questions helps mitigate cheating.)  In the third step, students
answer the questions. In the last step, the system grades each student
proportionally to her accuracy on assigned questions, i.e., by {\em
  simple averaging}.

While randomizing questions and grading with simple averaging is ex
ante fair, it is not generally ex post fair.  When questions in the
question bank have varying difficulty then by random chance a student
could be assigned more easy questions than average or more hard
questions than average.  Ex post in the random assignment of questions
to students, the simple averaging of scores on each question allows
variation in question difficulties to manifests as ex post
unfairness in the final grades.

The aim of this paper is to understand grading algorithms that are fair
and accurate.  Given a bank of possible questions, a benchmark for
both fairness and accuracy is the counterfactual grade that a student
would get if the student was asked all of the questions in the
question bank.  Exams that ask fewer questions to the students may be
inaccurate with respect to this benchmark and the inaccuracy may vary
across students and this variation is unfair.  This benchmark allows
for both the comparison of grading algorithms and the design of randomized
exams, i.e., the method for deciding which questions are asked to
which students.

The grading algorithms developed in this paper are based on the
Bradley-Terry-Luce model \citep{Bradley1952-nz} on bipartite
student-question graphs.  This model is also studied in the psychology
literature where it is known as the Rasch model
\citep{raschProbabilisticModelsIntelligence1993}.  This model views
the student answering process as a noisy comparison between a
parameter of the student and a parameter of the
question. Specifically, there is a merit value vector $u$ which describes
the student abilities and question difficulties and is unknown to
the instructor. The probability that student $i$ answers
question $j$ correctly is defined to be
\[f(u_i-u_j)=\frac{\exp(u_i)}{\exp(u_i)+\exp(u_j)},\]
where $f(x)=\frac{1}{1+\exp(-x)}$, and $u_i$, $u_j$ represents the merit value of student $i$ and question $j$ respectively.

The paper develops a grading algorithm that is based on the maximum
likelihood estimator $\boldsymbol{u^*}$ of the merit vector. The exam
result can be represented by a directed graph, where an edge from a
student to a question represents a correct answer and the opposite
direction represents an incorrect answer.  We prove that the maximum
likelihood estimator exists and is unique within a strongly connected
component (\Cref{thm:equiv}). Thus we use $f(u^*_i-u^*_j)$ to predict
the probability that the missing edge goes from student $i$ to
question $j$ within the same component. For missing edges across
comparable components, since all directed path between the vertices
have same directions, we predict a determined correct or incorrect
answer consistently with the path direction. For remaining edges, we
extend the heuristic of simple averaging.  Compared to simple
averaging which only focuses on student in-degrees and out-degrees, our
grading algorithm incorporates more structural information of the exam
result and, as we show, reduces ex post bias.

\paragraph{Results.}

Our theoretical analysis considers a sequence of distributions over
random question assignment graphs indexed by $n$ by setting the number of
students and number of questions in the question bank to $n$ and
assigning $d_n$ random questions uniformly and independently to each
student. Let $\alpha_n=\max_{1\leq i,j\leq 2n} u_i-u_j$ be the largest
difference between any pair of merits.  We prove that if
 \[\frac{\exp(\alpha_n)\log n}{d_n}\to 0\quad(n\to\infty),\]
then the probability that the exam result graph is strongly connected goes to 1 (\Cref{thm:connectivity}). Thus, the existence and the uniqueness of the MLE is guaranteed under the model. We also prove that if
\begin{equation}
    \exp\left(2(\alpha_n+1)\right)\sqrt{\frac{\log^3 n}{d_n\log^2 d_n}}\rightarrow 0\quad(n\rightarrow\infty),
\end{equation}
then the MLEs are uniformly consistent, i.e.,
$\|\boldsymbol{u}^*-\boldsymbol{u}\|_\infty\stackrel{\mathbb{P}}{\longrightarrow}
0$.  These theoretical results complement the empirical and simulation
results in the literature on the Rasch model with random missing data.  Our analysis is similar
to that of \citet{hanAsymptoticTheorySparse2020} which studies
Erd\"os-R\'enyi random graphs.


Our empirical analysis considers a study of grading algorithms on both
anonymous exam data and numerical simulations.  The exam data set
consists of 22 questions and 35 students with all students answering
all questions.  From this data set, randomized exams with fewer than 22
questions can be empirically studied and grading algorithms can be
compared.  Our algorithm outperforms simple averaging when students
are asked at least seven questions.  We fit the model parameters
to this real-world dataset and run numerical simulation with the
resulting generative model.  These simulations allow empirical
estimation of the ex post bias of our algorithm in comparison to
simple averaging.  For example, when each of 35
students answers a random 10 of the 22 questions, we find that the
maximum bias of simple averaging is more than ten times higher than
the maximum bias of our algorithm.  Specifically, the maximum bias of
any student for simple averaging is 13\% while the bias of our
algorithm is 1\%.

We evaluate a simple question of exam design via simulation.  Given an
infinite question bank, we sample a fixed number of active questions,
then we create a randomized exam with five questions for each
student drawn from this fixed number of active questions.  When there
are only five active questions our grading algorithm and simple averaging
coincide as all students are asked all active questions.  When there
are an infinite number of active questions the algorithms again
coincide as no two students are asked the same question and our
algorithm and simple averaging are the same.  By simulation we
consider the bias as a function of the number of active questions and
find that the optimal number of questions is about six to nine for maximum bias
and about 10 to 15 for average bias.

\paragraph{Illustrative Example.}


\Cref{fig:example} illustrates the unfairness that can arise in simple
averaging and the intuition for how our algorithm improves fairness.
In the fair exam grading problem, the instructor first assigns
questions to students according to an undirected student-question
bipartite graph, a.k.a., the task assignment graph
(\Cref{fig:example:assignment}).  The exam result can be represented
by a directed student-question bipartite graph, a.k.a., the exam
result graph (\Cref{fig:example:result}), where a directed edge from a
student to a question represents a correct answer and an opposite
direction represents an incorrect answer. Given the exam result graph,
the instructor uses a grading algorithm to estimate the average
accuracy of students on the whole question bank.

We take student S2 as an example to see how simple averaging, as one
specific grading rule, grade students
(\Cref{fig:example:averaging}). Simple averaging observes that student
S2 has one correct answer and one incorrect answer, in other words,
the corresponding vertex has in-degree one and out-degree one. Thus
simple averaging predicts that the probability of student S2 answering
the remaining question Q3 correctly is 0.5. The reason we believe 0.5
is not a good prediction is, in this exam, every student assigned
question Q3 answers it correctly, including student S5 and S6, who
give incorrect answers to question Q2.  We can infer that Q3 is a
relatively easy question. On the other hand, student S2 who can answer
question Q2 correctly has a relatively higher ability among the
class. Therefore, it is reasonable to believe that student S2 can give
a correct answer to question Q3 and, thus, simple averaging
underestimates her grade.

We show how our algorithm analyze the missing edge between student S2
and question Q3 in this example (\Cref{fig:example:my}).  Our
algorithm finds that student S2 belongs to the strongly connected
component \{S1,S2,Q1,Q2\}, while question Q3 belongs to \{Q3\} and the
missing edge goes across two comparable components. As a property of
the graph, any directed path between student S2 and question Q3 goes
from the student to the question. Our grading rule takes it as a
strong evidence of the S2's ability higher than Q3's difficulty
and predicts that student S2 can answer question Q3 correctly with
probability one.

\begin{figure}[!h]
    \subfigure[Task Assignment Graph]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \input{Figs/IntroEg/Assignment}
            \label{fig:example:assignment}
        \end{minipage}
    }\hfill
    \subfigure[Exam Result Graph]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \input{Figs/IntroEg/Result}
            \label{fig:example:result}
        \end{minipage}
    }
    \subfigure[simple averaging]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \input{Figs/IntroEg/Averaging}
            \label{fig:example:averaging}
        \end{minipage}
    }\hfill
    \subfigure[Our method]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \input{Figs/IntroEg/My}
            \label{fig:example:my}
        \end{minipage}
    }
    \caption{A running example of the exam grading problem}
    \label{fig:example}
\end{figure}


==> Body/5_theory.tex <==
\section{Theory}\label{sec:theory}
In this section, we show several properties of our algorithm. Recall that the Bradley-Terry-Luce model describes the outcome of pairwise comparisons as follows. In a comparison between subject $i$ and subject $j$, subject $i$ beats subject $j$ with probability \[p_{ij}=\frac{\exp(u_i)}{\exp(u_i)+\exp(u_j)}=f(u_i-u_j),\] where $\boldsymbol{u}=(u_1\dots,u_{2n})$ represents the merit parameters of $2n$ subjects and $f(x)=\frac{1}{1+\exp(-x)}$. We consider the Bradley-Terry-Luce model under a family of random bipartite task assignment graphs $\mathcal{B}(n,d_n)$. Specifically, a task assignment graph $G(L\cup R, E)$ with $n$ vertices in each part is constructed by linking $d_n$ different random vertices in $R$ to each left vertex in $L$, which means $L$ is regular but $R$ is not.

Given a task assignment graph $G$, denote $A$ as its adjacency matrix. For any two subjects $i$ and $j$, the number of comparisons between them follows $A_{ij}\in\{0,1\}$. We define $A'_{ij}$ as the number of times that subject $i$ beats subject $j$, thus $A'_{ij}+A'_{ji}=A_{ij}=A_{ji}$. In other words, $A'$ is the adjacency matrix of the exam result graph $G'$. Based on the observation of $G'$, the log-likelihood function is
\begin{equation}
\mathcal L(\boldsymbol{u})=\sum_{1\leq i\neq j\leq 2n}A'_{ij}\log p_{ij}=\sum_{1\leq i\neq j\leq 2n}A'_{ij}\log f(u_i-u_j).
\label{eq:likelihood}
\end{equation}

Denote $\boldsymbol{u}^*=(u_1^*,u_1^*,\dots,u_{2n}^*)$ as the maximum likelihood estimators (MLEs) of $\boldsymbol{u}$. Since $\mathcal{L}$ is additive invariant,  w.l.o.g.\ we assume $u_1=0$ and set $u^*_1=0$. Since $(\log f(x))'=1-f(x)$ the likelihood equation can be simplified to
\begin{equation}\label{eq:likelihood:foc}
\sum_{j=1}^{2n} A'_{ij}=\sum_{j=1}^{2n} A_{ij}f(u_i^*-u_j^*),\forall~i.
\end{equation}

\subsection{Existence and Uniqueness of the MLEs}
\citet{zermeloBerechnungTurnierErgebnisseAls1929c} and \citet{fordSolutionRankingProblem1957} gave a necessary and sufficient condition for the existence and uniqueness of the MLEs in \eqref{eq:likelihood:foc}.

\paragraph{Condition A.}
For every two nonempty sets that form a partition of the subjects, a subject in one set has beaten a subject in the other set at least once.
\\

To provide an intuitive understanding of Condition A, we show its equivalence to the strong connectivity of the exam result graph $G'$.

\begin{theorem}
Condition A holds if and only if the exam result graph $G'$ is strongly connected.
\label{thm:equiv}
\end{theorem}
\begin{proof}
Condition A says that for any partition $(V_1, V_2)$ of the vertices $L\cup R$, there exists an edge from $V_1$ to $V_2$ and also an edge from $V_2$ to $V_1$. If $G'$ is strongly connected, Condition A directly holds by definition of strong connectivity. Otherwise, if $G'$ is not strongly connected, the condensation of $G'$ contains at least two SCCs. We pick one strongly connected component with no indegree as $V_1$ and remaining vertices as $V_2$, then there is no edge from $V_2$ to $V_1$, i.e., Condition A fails.
\end{proof}
\vbox{}

% Before showing that Condition A is satisfied under certain sparsity conditions, we first introduce some notation:
% \begin{equation}
% \begin{split}
%     \alpha_n=\max_{0\leq i,j\leq 2n} u_i-u_j,\quad \Delta u_i=u_i-u^*_i\quad \text{and}\quad \Delta_n=??????,
% \end{split}
% \label{thm:connectivity:notation}
% \end{equation}
% where $\alpha_n$ is the largest difference between all possible pair of merits.

\begin{theorem}[Existence and Uniqueness of MLEs]
If
\begin{equation}
\frac{\exp(\alpha_n)\log n}{d_n}\rightarrow 0\quad (n\rightarrow\infty),    
\label{condition:connectivity}
\end{equation}
where $\alpha_n=\max_{1\leq i,j\leq 2n} u_i-u_j$ is the largest difference between all possible pair of merits, then $\Pr\left[\text{Condition A is satisfied}\right]\rightarrow 1\quad (n\rightarrow\infty).$
\label{thm:connectivity}
\end{theorem}

To prove Theorem $\ref{thm:connectivity}$, we first show the edge expansion property of the task assignment graph $G$ then bound the probability that $G'$ fails Condition A given the edge expansion property.

\begin{lemma}[Edge Expansion]
Under condition \eqref{condition:connectivity},
\[\Pr\left[\forall S\subset V,~\text{s.t.}~|S|\leq n,\quad \frac{|\partial S|}{|S|} > \frac{d_n}{4}\right]\rightarrow 1\quad (n\rightarrow\infty),\]
where $\partial S=\{(u,v)\in E:u\in S, v\in V\setminus S\}$ for the task assignment graph $G(V,E)$.
\label{thm:edge-expansion}
\end{lemma}
\begin{proof}
Consider any subset of vertices $S$ with size $r\leq n$.
Denote $X=S\cap L, Y=S\cap R, |X|=x$, thus $|Y|=r-x, |L\setminus X|=n-x, |R\setminus Y|=n+x-r$. $\partial S$ is a random variable that can be expressed as
\[|\partial S|=\sum_{u\in X}\sum_{v\in R\setminus Y}A_{uv}+\sum_{u\in L\setminus X}\sum_{v\in Y}A_{uv},\]
where $A$ is the adjacency matrix of the task assignment graph $G$.
Recall that the task assignment graph $G$ is generated by linking $d_n$ random different vertices in $R$ to each vertex in $L$. Thus for different $u_1\neq u_2\in L$, $A_{u_1\cdot}$ is independent with $A_{u_2\cdot}$, while for a fixed $u\in L$, $A_{u\cdot}$ is chosen randomly without replacement. Chernoff bound applies under such conditions, i.e.,
\[\Pr\left[|\partial S|\leq \frac{1}{2}\E\left[|\partial S|\right]\right]\leq \exp\left(-\frac{\E[|\partial S|]}{8}\right).\]
Then we lower bound $\E[|\partial S|]$ by
\begin{equation*}
\begin{aligned}
\E[|\partial S|]
&=\frac{d_n}{n}(|X||R\setminus Y|+|L\setminus X||Y|)\\
&=\frac{d_n}{n}(2x^2-2xr+nr)\geq \frac{d_n}{n}\left(-\frac{1}{2}r^2+nr\right)\geq \frac{d_nr}{2}.
\end{aligned}
\end{equation*}
Thus for any fixed set $S$ with size $r$,
\[\Pr\left[|\partial S|\leq \frac{d_nr}{4}\right]\leq \Pr\left[|\partial S|\leq \frac{1}{2}\E\left[|\partial S|\right]\right]\leq \exp\left(-\frac{\E[|\partial S|]}{8}\right)\leq \exp\left(-\frac{d_nr}{16}\right).\]
Finally, by union bound,
\begin{equation*}
\begin{aligned}
    \Pr\left[\forall S\subset V,~\text{s.t.}~|S|\leq n,\quad \frac{|\partial S|}{|S|} > \frac{d_n}{4}\right]
    &=1-\Pr\left[\exists S\subset V,~\text{s.t.}~|S|\leq n,\quad \frac{|\partial S|}{|S|} \geq  \frac{d_n}{4}\right]\\
    &\geq 1-\sum_{r=1}^n\binom{2n}{r}\exp\left(-\frac{d_nr}{16}\right)\\
    &\geq 1-\sum_{r=1}^n\exp\left(-\frac{d_nr}{16}+r\log(2n)\right)\\
    &\geq 1-\sum_{r=1}^n\exp\left(-\frac{d_nr}{48}\right)\\
    &\geq 1-\exp\left(-\frac{d_n}{48}+\log n\right)\\
    &\geq 1-\exp\left(-\frac{d_n}{192}\right)\\
\end{aligned}
\end{equation*}
The third-to-last inequality holds when $d_n>24\log(2n)$ and the last inequality holds when $d_n>64\log n$. Note that condition $\eqref{condition:connectivity}$ implies $\log n/d_n\rightarrow 0\quad (n\rightarrow\infty)$ since $\alpha_n\geq 0$. Thus for large enough $n$ and $d_n$,
\begin{equation*}
    \Pr\left[\forall S\subset V,~\text{s.t.}~|S|\leq n,\quad \frac{|\partial S|}{|S|} > \frac{d_n}{4}\right]\geq 1-\exp\left(-\frac{d_n}{192}\right)\rightarrow 1\quad (n\rightarrow\infty).
\end{equation*}
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:connectivity}]
For an edge between vertex $i$ and $j$ in the task assignment graph $G$, i.e. $A_{ij}=1$, the corresponding directed edge in the exam result graph $G'$ goes from $i$ to $j$ with probability 
\[\Pr[A'_{ij}=1]=f(u_i-u_j)\leq \max_{1\leq i,j\leq 2n} f(u_i-u_j)\leq \frac{1}{1+\exp(-\alpha_n)}\leq 2^{-\exp(-\alpha_n)}.\]
By Lemma \ref{thm:edge-expansion}, under condition \eqref{condition:connectivity},
\[\Pr\left[\forall S\subset V,~\text{s.t.}~|S|\leq n,\quad \frac{|\partial S|}{|S|} > \frac{d_n}{4}\right]\rightarrow 1\quad (n\rightarrow\infty).\]
Now consider any subset of vertices $S\subset V~\text{s.t.}~|S|=r\leq n$. The probability that all edges between $S$ and $V\setminus S$ go in the same direction in $G'$ is no more than $2\left(2^{-\exp(-\alpha_n)}\right)^{d_nr/4}$. Thus by union bound, the probability that Condition A holds is at least
\begin{equation*}
\begin{aligned}
    &1-2\sum_{1\leq r\leq n}\binom{2n}{r}\left(2^{-\exp(-\alpha_n)d_nr/4}\right)\\
    \geq &  1-2\left(\sum_{0\leq r\leq 2n}\binom{2n}{r}\left(2^{-\exp(-\alpha_n)d_nr/4}\right)-1\right)\\
    \geq & 1-2\left(\left(1+\left(2^{-\exp(-\alpha_n)d_n/4}\right)\right)^{2n}-1\right),\\
\end{aligned}
\end{equation*}
which converges to 1 when $n\rightarrow \infty$ under condition $\eqref{condition:connectivity}$.
\end{proof}

\subsection{Uniform Consistency of the MLEs}
Based on condition \eqref{condition:connectivity}, Theorem \ref{thm:connectivity} shows the existence and uniqueness of the MLEs. We will only discuss the situation when condition \eqref{condition:connectivity} is satisfied. In this part, we will prove the uniform consistency of the MLEs.

\begin{theorem}[Uniform Consistency of MLEs]
If
\begin{equation}
    \exp\left(2(\alpha_n+1)\right)\Delta_n\rightarrow 0\quad(n\rightarrow\infty),
    \label{condition:consistency}
\end{equation}
where $\Delta_n= \sqrt{\frac{\log^3 n}{d_n\log^2 d_n}}$, then the MLEs are uniformly consistent, i.e., $\|\boldsymbol{u}^*-\boldsymbol{u}\|_\infty\stackrel{\mathbb{P}}{\longrightarrow} 0$.
\label{thm:consistency}
\end{theorem}

Here we first provide a high-level description of the proof.
Denote $\varepsilon_i=u^*_i-u_i$ as the estimation error of the maximum likelihood estimators.
Since we assume $u_1=0$ and set $u_1^*=0$, we have $\varepsilon_1=u^*_1-u_1=0$.
Consider the two subjects with the most negative estimation error and the most positive estimation error
\[\lowelement=\mathop{\arg\min}\limits_i \varepsilon_i\leq \varepsilon_1=0\quad \text{and}\quad \highelement = \mathop{\arg\max}\limits_i \varepsilon_i\geq \varepsilon_1=0,\]
and their corresponding error
\[\loweps=\min\limits_i \varepsilon_i\quad \text{and}\quad \higheps = \max\limits_i \varepsilon_i,\]
then we have
\[\|\boldsymbol{u}^*-\boldsymbol{u}\|_\infty=\max\{-\loweps,\higheps\}\leq \higheps-\loweps.\]
Thus instead of directly proving $\|\boldsymbol{u}^*-\boldsymbol{u}\|_\infty\to 0$, we sufficiently bound the difference of $\higheps$ and $\loweps$.

The target of the proof is to identify a specific number $D$, such that there are more than half subjects satisfying that their estimation errors are no more than $\loweps+D$, and more than half subjects satisfying that their estimation errors are no less than $\higheps-D$. If we find such a number $D$, there will be at least one common subject in both sides, thus we can bound $\higheps-\loweps$ by $2D$. To identify the number, we will check a sequence of increasing numbers $\{D_k\}_{k=0}^{K_n}$, and the two corresponding growing sets $\{\lowset_k\}_{k=0}^{K_n}$ and $\{\highset_k\}_{k=0}^{K_n}$ that contains the subjects with estimation errors $D_k$-close to $\loweps$ and $\higheps$ respectively. Under careful choice of $K_n$ and $\{D_k\}_{k=0}^{K_n}$, we will show that $\lowset_{K_n}$ and $\highset_{K_n}$ both contain more than half subjects.

The main difficulty of the proof is to demonstrate the growth of $\{\lowset_k\}_{k=0}^{K_n}$ and $\{\highset_k\}_{k=0}^{K_n}$. We prove by considering the local growth of the sets, i.e., $N(\lowset_k)\cap \lowset_{k+1}$ and $N(\highset_k)\cap \highset_{k+1}$. By symmetry, we take $\lowset_k$ as an example to show the proof sketch. Specifically, \Cref{thm:vertex-expansion} analyze the generation of the random task assignment graphs and show a vertex expansion property that describes the growth of the neighborhoods $N(\lowset_k)$. \Cref{thm:local-property} starts with any vertex $i$ in $\lowset_k$, analyzes the first order equations to exclude the vertices that are in the neighborhoods $N(\{i\})$ and but are not in $\lowset_{k+1}$, and gives a lower bound on the size of $N(\{i\})\cap \highset_{k+1}$. Finally, we jointly consider all vertices in $\lowset_k$ and provide a lower bound on the size of $N(\lowset_k)\cap \lowset_{k+1}$, which finishes the proof.

Now we start our proof by introducing several notations
\begin{equation*}
\begin{aligned}
    &K_n = \left\lfloor\frac{2\log n}{\log d_n}+1\right\rfloor,\quad c_n = \frac{\exp(-(\alpha_n+1))}{4},\quad q_n=\frac{c_n\log d_n}{4\log n},\quad z_n=\sqrt{\frac{32\log n}{d_n}},\\
\end{aligned}
\end{equation*}
where $K_n$ defines number of steps of the growth, $c_n$ is a lower bound on $f'(x)$ for $|x|\leq \alpha_n+1$, $q_n$ is a lower bound on the local growth rate of $|N(\{i\}\cap \lowset_{k+1})|$ w.r.t. $|N(\{i\})|$, and $z_n$ is the deviation in the Chernoff bound we will use. The sequence of numbers $\{D_k\}_{k=0}^{K_n}$ is set to be
\begin{equation*}
\begin{aligned}
&D_k=\frac{4k}{c_n}\sqrt{\frac{2(1+z_n)\log n}{(1-z_n)d_n}}\quad \text{for}~k=0,1,\dots,K_n-1,\\
&D_{K_n}=\frac{80K_n}{c_n^2}\sqrt{\frac{2(1+z_n)\log n}{(1-z_n)d_n}},
\end{aligned}
\end{equation*}
and the two growing sets $\{\lowset_k\}_{k=0}^K$ and $\{\highset_k\}_{k=0}^K$ which contains the subjects with estimation error $D_k$-close to $\loweps$ and $\higheps$ respectively are defined as
\begin{equation*}
\begin{aligned}
&\lowset_k=\{j:\varepsilon_j-\loweps\leq D_k\}\\
&\highset_k=\{j:\higheps-\varepsilon_j\leq D_k\}.
\end{aligned}
\end{equation*}

Before starting proving the vertex expansion property of the task assignment graph $\mathcal{B}(n,d_n)$, we first bound the vertex degree by Chernoff bound and union bound,
\begin{equation}\label{thm:degree}
\forall~i\in V,\quad \Pr\left[(1-z_n)d_n\leq \left|N(\{i\})\right|\leq (1+z_n)d_n\right]\geq  1-n^{-4},
\end{equation}
where $z_n$ is defined above as $\sqrt{\frac{32\log n}{d_n}}$ that tends to 0 when $n\rightarrow\infty$ under condition \eqref{condition:connectivity}.

\begin{lemma}[Vertex Expansion]
Regarding the task assignment graph $G(L\cup R,E)\sim\mathcal B(n,d_n)$, for a fixed subset of vertex in the left part $X\subset L$ with $|X|\leq \frac{n}{2}$, it holds with probability $1-n^{-4|X|}$ that
\begin{itemize}
    \item If $1\leq |X|<n/d_n$,
    \[\frac{|N(X)|}{|X|}>(1-z_n)\left(1-\frac{d_n|X|}{n}\right)d_n;\]
    \item  If $|X|\geq n/d_n$,
    \[\frac{|N(X)|}{n}>1-z_n-e^{-1},\]
\end{itemize}
where $z_n=\sqrt{\frac{32\log n}{d_n}}$. Similar arguments exist for a fixed subset of vertex in the right part $Y\subset R$.
\label{thm:vertex-expansion}
\end{lemma}

\begin{proof}
We need to define another family of random bipartite graph $\tilde{\mathcal B}$. Each graph in $\tilde{\mathcal B}(n,d_n)$ contains $n$ vertices in each part and assigns $d_n$ random neighbors to each vertex in the left part (multi-edges are allowed). For any $X\subset L$, it's easy to see that $|N(X)|$ in $G\sim \mathcal B(n,d_n)$ stochastically dominates $|N(X)|$ in $G\sim\tilde{\mathcal B}(n,d_n)$. Thus it's sufficient to prove the theorem under $\tilde {\mathcal B}(n,d_n)$. On the other hand, counting $|N(X)|$ under $\tilde{\mathcal B}(n,d_n)$ is the same random process as counting the number of non-empty bins after independently throwing $d_n|X|$ balls u.a.r.\ into $n$ bins.
By linearity of expectation over every bin, we know
\[\E[|N(X)|]=n\left(1-\left(1-\frac{1}{n}\right)^{d_n|X|}\right).\]
We need several lower bounds of $\E[|N(X)|]$ here. With the fact of
\[\frac{x}{2}\leq 1-\exp(-x)\leq x,\quad \forall~0\leq x<1,\]
we have
\begin{equation*}
\begin{aligned}
\E[|N(X)|]=n\left(1-\left(1-\frac{1}{n}\right)^{d_n|X|}\right)\geq n\left(1-\exp\left(\frac{d_n|X|}{n}\right)\right)\geq \frac{d_n|X|}{2}.
\end{aligned}
\end{equation*}
Therefore, using Azuma's inequality, we can lower bound $|N(X)|$, i.e.,
\[\Pr\left[|N(X)|\leq (1-z_n)\E[|N(X)|]\right]
\leq \exp\left(-\frac{z_n^2\left(\E[|N(X)|]\right)^2}{2d_n|X|}\right)
= \exp\left(-\frac{z_n^2d_n|X|}{8}\right) \leq n^{-4|X|}.\]
Also, when $|X|<n/d_n$, we have
\[
\left(1-\left(1-\frac{1}{n}\right)^{d_n|X|}\right)\geq \frac{d_n|X|}{n}\left(1-\frac{d_n|X|}{n}\right),
\]
thus with probability $1-n^{-4|X|}$,
\[|N(X)|\geq (1-z_n)\E[|N(X)|]\geq (1-z_n)d_n|X|\left(1-\frac{d_n|X|}{n}\right);
\]
Similarly when $|X|\leq n/d_n$ , we have
\[
\left(1-\left(1-\frac{1}{n}\right)^{d_n|X|}\right)\geq 1-e^{-1},
\]
and
\[|N(X)|\geq (1-z_n)\E[|N(X)|]\geq (1-z_n)\left(1-e^{-1}\right)n\geq \left(1-z_n-e^{-1}\right)n.
\]
The proof for $Y\subset R$ is almost the same except that it's sufficient to use Chernoff bound rather than Azuma's inequality since the independence among the subjects in $N(Y)$.
\end{proof}

Lemma \ref{thm:vertex-expansion} describes the vertex expansion, an important structural property we need, of the task assignment graph $G$. In the next step, we will analyze the first order conditions \eqref{eq:likelihood:foc} and show a local property of $\lowset_k$. More specifically, Lemma \ref{thm:local-property} cares about for any subject in $\lowset_k$, how many of its neighbors are in $\lowset_{k+1}$.
\begin{lemma}[Local Growth of $\lowset_k$]
For $n$ large enough, round $k<K_n$ and a fixed subject $i\in \lowset_k$, it holds with probability $1-3n^{-4}$ that
\begin{itemize}
    \item If $k<K_n-1$,
            \[|N(\{i\})\cap \lowset_{k+1}|\geq q_n|N(\{i\})|,\]
            where $q_n=\frac{c_n\log d_n}{4\log n}$ and $c_n=\frac{\exp(-(\alpha_n+1))}{4}$;
    \item If $k=K_n-1$,
            \[|N(\{i\})\cap \lowset_{k+1}|\geq \frac{75}{81}|N(\{i\})|.\]
\end{itemize}
\label{thm:local-property}
\end{lemma}

\begin{proof}
Pick a subject $i\in \lowset_k$. From \eqref{thm:degree} we know that with probability $1-n^{-4}$,
\[(1-z_n)d_n\leq \left|N(\{i\})\right|\leq (1+z_n)d_n,\]
where $z_n=\sqrt{\frac{32\log n}{d_n}}$. For any task assignment graph $G$ and its adjacency matrix $A$, the corresponding adjacency matrix $A'$ of the exam result graph is a random variable of $A$. Specifically, for any $A_{ij}=1$, $A_{ij}'$s are independent Bernoulli random variables with probability $f(u_i-u_j)$ to be 1. In other words, $\E[A_{ij}']=A_{ij}f(u_i-u_j)$. By Chernoff bound,
\[\Pr\left[\left|\sum_j A_{ij}'-\sum_jA_{ij}f(u_i-u_j)\right|\geq \sqrt{2(1+z_n)d_n\log n}\right]\leq 2\exp\left(-\frac{4(1+z_n)d_n\log n}{|N(i)|}\right)\leq 2n^{-4}.\]
Thus according to equation \eqref{eq:likelihood:foc}, we have, with probability $1-3n^{-4}$,
\[\left|\sum_j A_{ij}\left(f(u_i-u_j)-f(u_i^*-u_j^*)\right)\right|<\sqrt{2(1+z)d_n\log n}.\]
Below we use the above inequality and some analysis of function $f$ to count the number of subjects in $N(\{i\})\cap \lowset_{k+1}$. The fact we use about function $f$ is
\begin{equation*}
\begin{aligned}
    & f'(x)=\frac{\exp(-x)}{(1+\exp(-x))^2}\leq \frac{1}{4}\quad \text{and}\\
    &f'(x)\geq \frac{\exp(-(\alpha_n+1))}{(1+\exp(-(\alpha_n+1)))^2}\geq \frac{\exp(-(\alpha_n+1))}{4}=c_n,~\forall|x|\leq \alpha_n+1.
\end{aligned}
\end{equation*}
Thus for another subject $j$ such that $\varepsilon_j \leq \varepsilon_i$, by mean value theorem, we have
\[f\left(u_i^*-u_j^*\right)-f\left(u_i-u_j\right)=f'(\xi_{ij})\left(\varepsilon_i-\varepsilon_j\right)\leq \frac{1}{4}\left(\varepsilon_i-\loweps\right)\leq \frac{D_k}{4},\]
where $\xi_{ij}\in\left[u_i-u_j,u_i^*-u_j^*\right]$. Similarly, for a subject $j$ with $\varepsilon_j > \varepsilon_i + D_{k+1}-D_k$, we have
\[f\left(u_i-u_j\right)-f\left(u_i^*-u_j^*\right)=f'(\xi'_{ij})\left(\varepsilon_j-\varepsilon_i\right)\geq c_n(D_{k+1}-D_k),\]
where $\xi'_{ij}\in\left[u_i^*-u_j^*,u_i-u_j\right]$. Since
\[u_i-u_j-D_{K_n}\leq u_i-u_j - \left(\varepsilon_j-\varepsilon_i\right)=u_i^*-u_j^* \leq \xi'_{ij}\leq u_i-u_j,\]
and $D_{K_n}\rightarrow 0$ as $(n\rightarrow\infty)$ under condition \eqref{condition:consistency}, $|\xi'_{ij}|$ is bounded by $\alpha_n+1$ when $n$ is large enough, thus $f'(\xi'_{ij})\geq c_n$. Therefore, on the one hand,
\begin{equation}
\begin{aligned}
& \sum_{u_j^*-u_j>u_i^*-u_i}A_{ij}\left(f(u_i-u_j)-f(u_i^*-u_j^*)\right)\\
= &\sum_{j}A_{ij}\left(f(u_i-u_j)-f(u_i^*-u_j^*)\right) - \sum_{u_j^*-u_j\leq u_i^*-u_i}A_{ij}\left(f(u_i-u_j)-f(u_i^*-u_j^*)\right)\\
\leq & \sqrt{2(1+z)d_n\log n} + \frac{1}{4}D_k\sum_{u_j^*-u_j\leq u_i^*-u_i}A_{ij}.
\end{aligned}
\label{thm:local:part1}
\end{equation}
On the other hand,
\begin{equation}
\begin{aligned}
& \sum_{u_j^*-u_j>u_i^*-u_i}A_{ij}\left(f(u_i-u_j)-f(u_i^*-u_j^*)\right)\\
\geq & \sum_{u_j^*-u_j> u_i^*-u_i+D_{k+1}-D_k}A_{ij}\left(f(u_i-u_j)-f(u_i^*-u_j^*)\right)\\
\geq & c_n(D_{k+1}-D_{k})\sum_{u_j^*-u_j> u_i^*-u_i+D_{k+1}-D_k}A_{ij}.
\end{aligned}
\label{thm:local:part2}
\end{equation}
Combining \eqref{thm:local:part1} and \eqref{thm:local:part2}, we have 
\[|N(\{i\})\cap \lowset_{k+1}|\geq \sum_{u_j^*-u_j\leq u_i^*-u_i+D_{k+1}-D_k} A_{ij}\geq \frac{c_n(D_{k+1}-D_k)-\sqrt{\frac{2(1+z_n)\log n}{(1-z_n)d_n}}}{c_n(D_{k+1}-D_k)+\frac{1}{4}D_k}|N(\{i\})|.\]
For $k<K_n-1$,
\[\frac{c_n(D_{k+1}-D_k)-\sqrt{\frac{2(1+z_n)\log n}{(1-z_n)d_n}}}{c_n(D_{k+1}-D_k)+\frac{1}{4}D_k}|N(\{i\})|\geq q_n|N(\{i\})|.\]
For $k=K_n-1$,
\[\frac{c_n(D_{k+1}-D_k)-\sqrt{\frac{2(1+z_n)\log n}{(1-z_n)d_n}}}{c_n(D_{k+1}-D_k)+\frac{1}{4}D_k}|N(\{i\})|\geq \frac{75}{81}|N(\{i\})|.\]
\end{proof}

With the help of Lemma \ref{thm:vertex-expansion} and \ref{thm:local-property}, we are able to show the growth from $\lowset_k$ to $\lowset_{k+1}$. Specifically, we consider two subsets of $\lowset_k$, $X_k=\lowset_k\cap L$ and $Y_k=\lowset_k\cap R$, and use the following inequalities
\begin{equation}
\begin{aligned}
|Y_{k+1}|\geq |N(X_k)\cap \lowset_{k+1}|&=|N(X_k)|-|N(X_k)\cap \overline{\lowset_{k+1}}|\\
&=|N(X_k)|-\sum_{i\in X_k}|N(\{i\})\cap \overline{\lowset_{k+1}}|\\
&=|N(X_k)|-\sum_{i\in X_k}\left(|N(\{i\})|-|N(\{i\})\cap \lowset_{k+1}|\right),\\
|X_{k+1}|\geq |N(Y_k)\cap \lowset_{k+1}|&=|N(Y_k)|-|N(Y_k)\cap \overline{\lowset_{k+1}}|\\
&=|N(Y_k)|-\sum_{i\in Y_k}|N(\{i\})\cap \overline{\lowset_{k+1}}|\\
&=|N(Y_k)|-\sum_{i\in Y_k}\left(|N(\{i\})|-|N(\{i\})\cap \lowset_{k+1}|\right),\\
\end{aligned}
\label{thm:consistency:fact}
\end{equation}
to show the growth of $X_k$ and $Y_k$ respectively.

\begin{proof}[Proof of Theorem \ref{thm:consistency}]
Denote $X_k=\lowset_k\cap L$ and $Y_k=\lowset_k\cap R$. We inductively prove the following fact that, for $n$ large enough, with probability $1-n^{-2}$,
\begin{itemize}
    \item For $1\leq k\leq K_n-2$,
        \[|X_k|,|Y_k|\geq d_n^{(k-1)/2};\]
    \item for $k = K_n-1$,
        \[|X_k|,|Y_k|\geq \frac{n}{d_n};\]
    \item for $k = K_n$,
        \[|X_k|,|Y_k|> \frac{n}{2}.\]
\end{itemize}

From now on we only consider $n$ large enough. Since $\lowelement\in \lowset_0$, w.l.o.g.\ we assume $|X_0|=1$. if $X_0$ contains other subjects, we take a subset with size 1. Then by fact \eqref{thm:consistency:fact}, \eqref{thm:degree} and Lemma \ref{thm:local-property}, we know with probability $1-4n^{-4}$ that
\[|Y_1|\geq |N(X_0)\cap \lowset_{k+1}|\geq q_n|N(X_0)|\geq q_n(1-z_n)d_n>0.\]
% we prove with probability $??$, for $|X_k|\leq n/d_n^{3/2}$, we have $|Y_{k+1}|\geq d^{1/2}|X_k|$. 
For $1<k\leq K_n-2$, we prove inductively. We assume $|X_k|=d_n^{(k-1)/2}$. If $X_k$ is larger, we pick any subset with size $d_n^{(k-1)/2}$. Fact \eqref{thm:consistency:fact} show that
\[
|Y_{k+1}|\geq |N(X_k)|-\sum_{i\in X_k}\left(|N(\{i\})|-|N(\{i\})\cap \lowset_{k+1}|\right).
\]
By Lemma \ref{thm:vertex-expansion} and union bound over all subset of $L$ with size $d_n^{(k-1)/2}$, it holds with probability $1-n^{-3|X_k|}$ that,
\[|N(X_k)|>(1-z_n)\left(1-\frac{d_n|X_k|}{n}\right)d_n|X_k|.\]
By Lemma\ref{thm:local-property} and union bound over all possible subject $i\in X_k$, it holds with probability $1-3n^{-3}$ that,
\[\forall i\in X_k,~|N(\{i\})\cap \lowset_{k+1}|\geq q_n|N(\{i\})|.\]
By \eqref{thm:degree} and union bound over all possible subject $i\in X_k$, it holds with probability $1-n^{-3}$ that,
\[\forall i\in X_k,~(1-z_n)d_n\leq |N(\{i\})|\leq (1+z_n)d_n.\]
Therefore, with probability $1-4n^{-3}$ we have
\begin{equation*}
\begin{aligned}
|Y_{k+1}|
&\geq |N(X_k)|-\sum_{i\in X_k}\left(|N(\{i\})|-|N(\{i\})\cap \lowset_{k+1}|\right)\\
&\geq |N(X_k)|-(1-q_n)\sum_{i\in X_k}|N(\{i\})|\\
&\geq (1-z_n)\left(1-\frac{d_n|X_k|}{n}\right)d_n|X_k|-(1-q_n)(1+z_n)d_n|X_k|\\
&\geq |X_k|d_n^{1/2}\left((1+z_n)q_nd_n^{1/2}-2z_nd_n^{1/2}-(1-z_n)\frac{d_n^{3/2}|X_k|}{n}\right)\\
&\geq |X_k|d_n^{1/2}\left(q_nd_n^{1/2}-2z_nd_n^{1/2}-\frac{d_n^{3/2}|X_k|}{n}\right)\\
&\geq |X_k|d_n^{1/2}\left(q_nd_n^{1/2}-2z_nd_n^{1/2}-1\right),
\end{aligned}
\end{equation*}
where the last inequality holds because we assume $|X_k|=d_n^{(k-1)/2}$, thus the last term satisfies \[d_n^{3/2}|X_k|/n=d_n^{(k+1)/2}/n\leq d_n^{(K_n-1)/2}/n\leq 1.\]
Finally, under condition $\eqref{condition:consistency}$, we have for large enough $n$, $q_nd_n^{1/2}-2z_nd^{1/2}-1>1$, which finishes the proof of the fact for $k\leq K_n-1$.
The proof for $k=K_n$ is similar with the help of the same lemmas and inequalities. Thus with probability $1-4n^{-3}$, for large enough $n$,
\begin{equation*}
\begin{aligned}
|Y_{K_n}|
&\geq |N(X_{K_n-1})|-\sum_{i\in X_{K_n-1}}\left(|N(\{i\})|-|N(\{i\})\cap \lowset_{K_n}|\right)\\
&\geq |N(X_{K_n-1})|-\left(1-\frac{75}{81}\right)\sum_{i\in X_{K_n-1}}|N(\{i\})|\\
&\geq (1-z_n-e^{-1})n-\frac{6}{81}(1+z_n)n\\
&> \frac{n}{2}.
\end{aligned}
\end{equation*}
The same proof applies for $|Y_{k}|$ and $|X_{k+1}|$. To summarize, with probability $1-n^{-2}$, $|X_{K_n}|,|Y_{k_n}|> n/2$, thus $|\lowset_{K_n}|> n$. By symmetry, $|\highset_{K_n}|>n$ with probability $1-n^{-2}$. Then with probability $1-2n^{-2}$, at least one subject $i\in \lowset_{K_n}\cap \highset_{K_n}$ lies in both $\lowset_{K_n}$ and $\highset_{K_n}$. By definition, subject $i$ satisfies
\[
\varepsilon_i-\loweps\leq D_{K_n}\quad \text{and}\quad 
\higheps-\varepsilon_i\leq D_{K_n},
\]
thus
\[\|\boldsymbol{u}^*-\boldsymbol{u}\|_\infty\leq \higheps-\loweps\leq 2D_{K_n},\]
which tends to 0 under condition \eqref{condition:consistency}.
\end{proof}

\subsection{Analysis of Our Algorithm}

Our algorithm uses the MLEs to predict the student's performance within the component. Based on the consistency of the MLEs, we show the bias of our algorithm when Condition A is satisfied.
\begin{theorem}
When Condition A is satisfied, the exam result graph is strongly connected. In this case, the MLE is unique and we have
\[
\left|\mathrm{alg}_i-\mathrm{opt}_i\right|\leq \frac{1}{2}\|\boldsymbol{u}-\boldsymbol{u}^*\|_{\infty}.
\]
\end{theorem}
\begin{proof}
When the exam result graph is strongly connected, the algorithm calculates the MLEs $\boldsymbol{u}^*$ and gives student $i$ a grade of $\mathrm{alg}_i=\frac{1}{|Q|}\sum_{j\in Q}f(u_i^*-u_j^*)$, while the ground truth probability of answering a random question correctly is $\mathrm{opt}_i=\frac{1}{|Q|}\sum_{j\in Q}f(u_i-u_j)$. Thus we have
\begin{equation}
\begin{aligned}
|\mathrm{alg}_i-\mathrm{opt}_i|
= &\left|\frac{1}{|Q|}\sum_{j}f(u_i^*-u_j^*)-\frac{1}{|Q|}\sum_{j}f(u_i-u_j)\right|\\
\leq &\frac{1}{|Q|}\sum_{j}\left|f(u_i^*-u_j^*)-f(u_i-u_j)\right|\\
= &\frac{1}{|Q|}\sum_{j}\left|f'(\xi_{ij})\right|\left|\varepsilon_i-\varepsilon_j\right|\\
\leq &\frac{2}{n}\|\boldsymbol{u}-\boldsymbol{u}^*\|_{\infty}\sum_{j}\left|f'(\xi_{ij})\right|\\
\leq &\frac{1}{2}\|\boldsymbol{u}-\boldsymbol{u}^*\|_{\infty},
\end{aligned}
\end{equation}
where the third-to-last equality is because of the mean value theorem, the next-to-last inequality is because $\left|\varepsilon_i-\varepsilon_j\right|\leq 2 \|\boldsymbol{u}-\boldsymbol{u}^*\|_{\infty}$, and the last inequality is because $|f'(x)|\leq \frac{1}{4}$.
\end{proof}
Next we discuss the performance of our algorithm on several extreme cases of the task assignment graph. For example, the extremely sparse cases when $N(i)$ is mutually disjoint for each student $i$ or each student receives only $d=1$ question. Another example is that the task assignment graph is a complete bipartite graph. In all of the above cases, our algorithm gives the same grade as simple averaging.

\begin{theorem}
When the task assignment graph satisfies that $N(i)$ is mutually disjoint for each student $i$ or each student receives only $d=1$ question, our algorithm gives the same grade as simple averaging.
\end{theorem}

\begin{proof}
In both cases, the exam result graph satisfies that every SCC is a single point, thus the algorithm's output totally relies on cross-component predictions. For each student, the comparable components for each student are exactly the questions that student receives. Thus the algorithm gives the same prediction as the student's correctness on those questions. The prediction for remaining questions is the average accuracy on the assigned questions by the algorithm's rule for incomparable components. Therefore, the algorithm's grade for the student is exactly the same as simple averaging.
\end{proof}

\begin{theorem}
When the task assignment graph is a complete bipartite graph, our algorithm gives the same grade as simple averaging.
\end{theorem}

\begin{proof}
In this case, the output of the algorithm only relies on existing edges. It directly follows that the algorithm gives the same grade as simple averaging.
\end{proof}

==> Body/6_experiments.tex <==
\section{Experiments}

\subsection{Real-World Data}
We collected the anonymous answer sheets from one exam with $|S|=35$ students and $|Q|=22$ questions. The task assignment graph of the exam is a complete bipartite graph, i.e., each student is assigned with all questions. The corresponding exam result graph is strongly connected, which means we can infer about student abilities and question difficulties under the Bradley-Terry-Luce model (\Cref{fig:complete-data:ecdf}).

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/complete-data/merit-value.pdf}
    \caption{Empirical Cumulative Distribution of Merit Value. We analyze all students and questions under the Bradley-Terry-Luce model and show the empirical cumulative density function of inferred student abilities and question difficulties. The abilities ranges from -1.486 to 1.149 while the difficulties ranges from -3.090 to 2.099.}
    \label{fig:complete-data:ecdf}
\end{figure}

\subsection{Algorithms}

\paragraph{Simple Averaging} The grade for student $i$ is its average correctness on assigned questions. See a formal definition in \Cref{example:Avg}.

\paragraph{Our Algorithm} The grade for student $i$ is an aggregation of the algorithm's prediction on her performance on each question. All predictions can be classified into four cases, including existing edges (keep the fact as prediction), same component (maximum likelihood estimators), comparable components (determined answer in line with the path direction) and incomparable components (heuristic as simple averaging).  See its formal definition in \Cref{sec:method:grading rule}.

\paragraph{Maximum a Posteriori Estimation} This algorithm maximizes the posterior probability or equivalently $\Pr[G'|G,\boldsymbol{u}]\Pr[\boldsymbol{u}]$, where $G'$ is the exam result graph, $G$ is the task assignment graph, $\boldsymbol{u}$ is the merit value vector and $\Pr[\boldsymbol{u}]$ is the prior distribution of $\boldsymbol{u}$. The prior distribution is defined to be a i.i.d. normal distribution on each merit value, where its mean and variance is fitted by the real-world data shown by \Cref{fig:complete-data:ecdf}. It then use the maximizer $\boldsymbol{u}^*$ to predict the missing edge between student $i$ and question $j$ by $f(u^*_i-u^*_j)$, where $f(x)=\frac{1}{1+\exp(-x)}$.

\subsection{Simulation 1: A Visualization of Simple Averaging's Ex-post Unfairness}\label{subsec:visual}
We compare the ex-post bias (\Cref{definition:ex-post bias}) between our algorithm and simple averaging given a fixed random task assignment graph. The simulation setting is the following. There are $|S|=35$ students and $|Q|=22$ questions, whose abilities and difficulties respectively are shown in \Cref{fig:complete-data:ecdf}. The task assignment graph is generated by \Cref{alg:graph} with the parameter $m=|Q|$ and $d=10$, i.e. each student is assigned 10 random questions from the whole question bank. The exam result graph is repeatedly generated according to the model.

\Cref{fig:fixed} shows the performance of two algorithms. The left plot corresponds to our algorithm and the right plot corresponds to simple averaging. In each plot, there are 35 confidence intervals, each corresponds to the difference between the student's expected grade and her benchmark, i.e. $\mathrm{alg}_i-\mathrm{opt}_i$. The confidence intervals in the left plot are significantly closer to 0, compared to the right plot, which visualizes the intuition that students are facing different overall question difficulties under the random assignments and simple averaging fails to adjust their grades. Instead, our algorithm infers the question difficulties and the student abilities and adjust their grades accordingly, thus could largely reduce the ex-post unfairness.

\begin{figure}[htbp]
    \centering
    \subfigure[Ex-post Grade Error of Our Algorithm]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/complete-data/g0-ConfidenceInterval_Ours.pdf}
        \end{minipage}
    }
    \subfigure[Ex-post Grade Error of Simple Averaging]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/complete-data/g0-ConfidenceInterval_Avg.pdf}
        \end{minipage}
    }
    \caption{A Visualization of the Ex-post Grade Error with Degree Constraint $d=10$}
    \label{fig:fixed}
\end{figure}

\subsection{Simulation 2: The Effect of the Degree Constraint}

We compare the expected maximum ex-post bias among students and the expected average ex-post bias among students between our algorithm (Ours) and simple averaging (Avg). The simulation setting is the following. There are $|S|=35$ students and $|Q|=22$ questions, whose abilities and difficulties respectively are showed in \Cref{fig:complete-data:ecdf}. For each degree constraint $d$, we repeatedly generate task assignment graphs using algorithm~\Cref{alg:graph} with the other parameter $m=|Q|$. For each task assignment graph, the exam result graph is repeatedly generated according to the model.

\Cref{fig:ex-post bias} shows two algorithms' expected maximum ex-post bias (\Cref{fig:ex-post bias:maximum}) and expected average ex-post bias (\Cref{fig:ex-post bias:average}) under different degree constraints. It can be seen that our algorithm (blue curve) outperforms simple averaging (red curve) on every degree constraint $d$. Our algorithm's expected ex-post bias with the degree constraint $d=6$ is close to simple averaging's with the degree constraint $d=20$, which means our algorithm can ask 14 less questions to each student to achieve a same grading accuracy as simple averaging.

\begin{figure}[htbp]
    \centering
    \subfigure[Expected Maximum Ex-post Bias]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/complete-data/MbiasCurve.pdf}
        \end{minipage}
        \label{fig:ex-post bias:maximum}
    }
    \subfigure[Expected Average Ex-post Bias]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/complete-data/AbiasCurve.pdf}
        \end{minipage}
        \label{fig:ex-post bias:average}
    }
    \caption{Expected Aggregated Ex-post Bias v.s. Degree Constraint}
    \label{fig:ex-post bias}
\end{figure}

If we zoom in on a specific degree constraint, we can see two algorithms' maximum ex-post bias and average ex-post bias on every different task assignment graph. \Cref{fig:random} shows the case with the degree constraint $d=10$. \Cref{fig:random:maximum} corresponds to the maximum ex-post bias and \Cref{fig:random:average} corresponds to the average ex-post bias. In each case, the left plot contains 100 points, corresponding to a different task assignment graph, whose x-axis is the aggregated ex-post bias of simple averaging and whose y-axis is that of our algorithm; the right plot is the histogram of the difference of the aggregated ex-post bias between our algorithm and simple averaging. The simulation results show that our algorithm has negligible aggregated ex-post bias compared to simple averaging on every task assignment graph.
\begin{figure}[!h]
    \centering
    \subfigure[Expected Maximum Ex-post Bias: 0.011 for Our Algorithm and 0.133 for Simple Averaging]{
        \begin{minipage}{0.8\linewidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/complete-data/MaximumBias.pdf}
        \end{minipage}
        \label{fig:random:maximum}
    }
    \subfigure[Expected Average Ex-post Bias: 0.004 for Our Algorithm and 0.047 for Simple Averaging]{
        \begin{minipage}{0.8\linewidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/complete-data/AverageBias.pdf}
        \end{minipage}
        \label{fig:random:average}
    }
    \caption{Aggregated Ex-post Bias on Task Assignment Graphs with Degree Constraint $d=10$}
    \label{fig:random}
\end{figure}


\subsection{Simulation 3: The Effect of the Question Sample Size}

We now consider the case where question bank is infinite and compare the expected maximum ex-post bias and the expected average ex-post bias between our algorithm and simple averaging. We sampled and fixed $|S|=5$ random students among the previous $35$ students. The question difficulties are i.i.d. distributed according to the linear interpolation of the difficulties shown in \Cref{fig:complete-data:ecdf}. For each question sample size $m$, we repeatedly generate task assignment graphs using \Cref{alg:graph} with the other parameter $d=5$. It can be expected that when $m=d$ and $m\to\infty$, two algorithms should have the same performance. \Cref{fig:infinite:small} shows a consistantly smaller expected maximum ex-post bias (\Cref{fig:infinite:small:maximum}) and expected average ex-post bias (\Cref{fig:infinite:small:average}) of our algorithm (blue curve) than simple averaging (red curve). As the question sample size grows, the expected aggregated ex-post bias of our algorithm first decreases and then increases. The turning point is about 6-9 for expected maximum ex-post bias and 10-15 for expected average ex-post bias.

\begin{figure}[htbp]
\centering
    \subfigure[Expected Maximum Ex-post Bias]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/infinite-question-bank/MaximumBiasCurve.pdf}
        \end{minipage}
        \label{fig:infinite:small:maximum}
    }
    \subfigure[Expected Average Ex-post Bias]{
        \begin{minipage}{0.45\linewidth}
            \centering
            \includegraphics[width=\textwidth]{Figs/infinite-question-bank/AverageBiasCurve.pdf}
        \end{minipage}
        \label{fig:infinite:small:average}
    }
    \caption{Expected Aggregated Ex-post Bias v.s. Question Sample Size}
    \label{fig:infinite:small}
\end{figure}



% \subsection{Model Cross Validation}
% We randomly split the real-world dataset into training data and test data. Specifically, each time we choose $d$ questions for each student and use the corresponding answers as the training data, use our algorithm and simple averaging to predict the outcome of each remaining student-question pair, and calculate the mean squared error (MSE). Formally, denote $X$ as the training set and $Y$ as the set of remaining student-question pairs, and the MSE in the model cross validation part is defined as \[\mathrm{MSE_{MCV}}=\E_{X,Y}\E_{(i,j)\sim\mathcal U(Y)}\left[\left(\mathrm{alg}_{ij}-w_{ij}\right)^2\right],\]
% where $\mathrm{alg}_{ij}=h_{ij}$ for our algorithm, and $\mathrm{alg}_{ij}$ equals to the average accuracy for student $i$ on the training set for simple averaging. We calculate the mean squared error $\mathrm{MSE_{MCV}}$ for each fixed degree $d=1\dots|Q|-1$. Figure~\ref{fig:MCV:MSECurve} shows the curve of $\mathrm{MSE_{MCV}}$ versus $d$. When the degree is at least 5, our algorithm has a smaller mean squared error and the advantage gets larger as the degree grows. The phenomenon could be explained by the result of model over-fitting in the low data environment, and the positive effects of merit parameters when we have enough data.

% We then consider the case when there are different number of students. Each time we randomly choose $d_1$ students, randomly assign $d_2$ questions to each student as the training set, use our algorithm and simple averaging to predict the outcome of the remaining student-question pair for the chosen students, and calculate the mean squared error. Formally the difference from the previous experiment is that $Y$ only consists the remaining student-question pairs where the student is chosen in this round. We know from the previous experiments that when training set is large enough, our algorithm performs better than simple averaging. In this experiments, we care about what the degree is when our algorithm performs better for a fixed student sample size. Figure~\ref{fig:MCV:Threshold} shows the degree threshold corresponding to the student sample size, i.e., for a student sample size $d_1$, if we set the degree $d_2$ at least the threshold, our algorithm has a smaller mean squared error than simple averaging.

% \begin{figure}[!h]
%     \subfigure[Mean Squared Error]{
%         \begin{minipage}{0.45\linewidth}
%             \centering
%             \includegraphics[width=\textwidth]{Figs/complete-data/MSECurve.png}
%             \label{fig:MCV:MSECurve}
%         \end{minipage}
%     }\hfill
%     \subfigure[Threshold]{
%         \begin{minipage}{0.45\linewidth}
%             \centering
%             \includegraphics[width=\textwidth]{Figs/complete-data/Threshold.png}
%             \label{fig:MCV:Threshold}
%         \end{minipage}
%     }
%     \caption{Model Cross Validation}
%     \label{fig:MCV}
% \end{figure}

% We can see a strange turning point in Figure~\ref{fig:MCV:MSECurve} that the curve once goes up when the degree is 4. We explain the reason below. Imagine the case where we have only two students and they are in the same SCC. Consider a question that is assigned to only one students, say student 1, our algorithm would predict that student 2 has the same outcome with student 1. The prediction comes from the ``Comparable Components'' part of our algorithm is too certain in such a low data environment. And when we increase the degree in this 2-student case, some missing edges in the ``Incomparable Components'' would turn into the case of ``Comparable Components'' thus increase the error. However, the prediction is reasonable if we have enough student and assign enough questions to each student, since it shows a different level of abilities or difficulties.

\subsection{Real-World Data Experiment: Cross Validation} We cannot repeat an exam in real world and check the ex-post bias of the algorithms. Thus, we sample part of the data we have as a new exam result, and use them to predict the students' actual average on the data. We randomly split the real-world data into training data and test data. Specifically, for a fixed student sample size $d_1$ and a degree constraint $d_2$, in each repetition, we randomly sample $d_1$ students and randomly choose $d_2$ questions and corresponding answers for each student as the training data, use our algorithm (Ours), simple averaging (Avg) and maximum a posteriori estimation (MAP) to predict every student's average accuracy on the whole question bank, and calculate the mean squared error. Formally, the mean squared error $\mathrm{MSE}$ is defined as
\[\mathrm{MSE}=\E_{X,\Tilde{S}}\left[\frac{1}{|\Tilde{S}|}\sum_{i\in \Tilde{S}}\left(\mathrm{alg}_{i}-\frac{1}{|Q|}\sum_{j\in Q}w_{ij}\right)^2\right],\]
where $X$ is the training set given a fixed degree $d$, $\Tilde{S}$ is the sampled student set, $\mathrm{alg}_i$ is student $i$'s grade given by the algorithm and $w_{ij}$ is the correctness of student $i$'s answer to question $j$.

In \Cref{fig:grading-rule:MSE}, we fix the student sample size $d_1 = |S|$, i.e., $\Tilde{S} = S$ and change the degree constraint $d_2$ from 1 to $|Q|$ and show the curve of the logarithmic of $\mathrm{MSE}$. Maximum a posteriori estimation as a regularized algorithm performs the best at a low data environment when the degree constraint $d_2$ is less than 12. Our algorithm performs better than simple averaging when the degree constraint $d_2$ is larger than 5 and has 16\% to 20\% smaller MSE compared to simple averaging when the degree constraint $d_2$ is larger than 10. In \Cref{fig:grading-rule:Threshold}, we consider for every possible student sample size $d_1$, what the smallest degree constraints $d_2$ is for our algorithm to perform better than simple averaging or maximum a posteriori estimation. It provides a reference for choosing the grading rule in different situations.

We additionally run a same cross validation in numerical simulation. We assume two different Normal prior distributions for student abilities and question difficulties, fitted by the data in \Cref{fig:complete-data:ecdf}. For a fixed student sample size $d_1$ and degree constraint $d_2$, in every repetition, we first draw $d_1$ i.i.d. student abilities and $|Q|=22$ i.i.d. question difficulties from those two prior distributions. We use a complete task assignment graph to generate the exam result graph according to the model. Then we randomly choose $d_2$ questions and the corresponding answers of each student as the training set, and use our algorithm, simple averaging and maximum a posteriori estimation to predict each student's average accuracy over the whole question bank. Note that we do exact same things in the cross validation, so when calculating the MSE, we compare the algorithms' grades to the students' average accuracy given by the exam result graph instead of the benchmark. From \Cref{fig:simulated grading-rule} we observe that the simulation result is quite similar to that of the real-world cross validation, which suggests that the numerical simulation result could be a good reference for the practical use of our algorithm.


\begin{figure}[!h]
    \centering
    \subfigure[Logarithmic of MSE v.s. Degree Constraint]{
        \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=0.98\textwidth]{Figs/complete-data/AggregatedLogMSECurve.pdf}
        \end{minipage}
        \label{fig:grading-rule:MSE}
    }
    \hfill
    \subfigure[Threshold v.s. Student Sample Size]{
        \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=0.98\textwidth]{Figs/complete-data/Threshold.pdf}
        \end{minipage}
        \label{fig:grading-rule:Threshold}
    }
    \caption{Cross Validation}
    \label{fig:grading-rule}
\end{figure}


\begin{figure}[!h]
    \centering
    \subfigure[Logarithmic of MSE v.s. Degree Constraint]{
        \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=0.98\textwidth]{Figs/complete-data/SimulatedAggregatedLogMSECurve.pdf}
        \end{minipage}
        \label{fig:simulated grading-rule:MSE}
    }
    \hfill
    \subfigure[Threshold v.s. Student Sample Size]{
        \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=0.98\textwidth]{Figs/complete-data/SimulatedThreshold.pdf}
        \end{minipage}
        \label{fig:simulated grading-rule:Threshold}
    }
    \caption{Simulated Cross Validation}
    \label{fig:simulated grading-rule}
\end{figure}


==> Body/7_conclusion.tex <==
\section{Conclusions}\label{sec:conclusion}

We formulate and study the fair exam grading problem under the
Bradley-Terry-Luce model. We propose an algorithm that is a
generalization of the maximum likelihood estimation method. To
theoretically validate our algorithm, we prove the existence,
uniqueness, and the uniform consistency of the maximum likelihood
estimators under the Bradley-Terry-Luce model on sparse bipartite
graphs. Our algorithm significantly outperforms simple averaging in
numerical simulation. On real-world data, our algorithm is better when
the students are assigned a sufficient number of questions (i.e., on
sufficiently long exams).  In the low-degree environment where the
students are assigned a small number of questions, we observe that the
maximum a posteriori estimation (with a fitted prior distribution),
which can be seen as a regularization of the maximum likelihood
estimation, performs the best. We provide guidelines for how to choose
the grading rule given certain number of students and a fixed exam
length.

Our model in this paper mainly considers true-or-false questions,
which can be extended to multiple choice questions and to the case
where it can be assumed that students would guess if they cannot solve
the question.  Our method to treat missing edges across comparable
components needs to be improved especially in the low-degree
environment (i.e., short exam lengths), since little information
across the components should not result in a determined prediction.
It is likely that our theoretical analysis can be extended to
scenarios where the number of students and the size of the question
bank are different.


==> Body/theory_ori.tex <==
\section{Theory}
The Bradley-Terry model describes the outcome of pairwise comparisons as follows. In a comparison between subject $i$ and subject $j$, subject $i$ beats subject $j$ with probability \[p_{ij}=\frac{u_i}{u_i+u_j},\] where $\boldsymbol{u}=(u_0,u_1\dots,u_{n})$ represents the merit parameters of $n+1$ subjects. In this section, we will mainly consider the consistency of the maximum likelihood estimator of the merit vector under the Bradley-Terry model, on any simple $d$-regular expanders.

Given a simple $d$-regular expander $G$, denote $A$ as its adjacency matrix. For any two subjects $i$ and $j$, the number of comparisons between them follows $A_{ij}\in\{0,1\}$. We define $a_{ij}$ as the number of times that subject $i$ beats subject $j$, thus $a_{ij}+a_{ji}=A_{ij}=A_{ji}$. The likelihood function is
\begin{equation}
\mathcal L(\boldsymbol{u})=\prod_{0\leq i\neq j\leq n}p_{ij}^{a_{ij}}=\frac{\prod_{0\leq i\leq n}u_i^{a_i}}{\prod_{0\leq i\neq j\leq n}(u_i+u_j)^{A_{ij}}},
\label{eq:likelihood}
\end{equation}where $a_i=\sum_{j=0}^n A_{ij}a_{ij}$. Denote $\boldsymbol{u}^*=(u_0^*,u_1^*,\dots,u_{n}^*)$ as the maximum likelihood estimators (MLEs) of $\boldsymbol{u}$. Since $\mathcal{L}$ is multiplicative invariant, we set $u^*_0=1$ as in \citet{simonsAsymptoticsWhenNumber1999}. The likelihood equation is
\begin{equation}\label{eq:likelihood:foc}
a_i=\sum_{j=0}^n \frac{A_{ij}u_i^*}{u_i^*+u_j^*},\forall~i.
\end{equation}


By \citet{zermeloBerechnungTurnierErgebnisseAls1929c} and \citet{fordSolutionRankingProblem1957}, the following Condition A ensures the existence and uniqueness of the MLEs in \eqref{eq:likelihood}.

\paragraph{Condition A.}
For every two nonempty sets that form a partition of the subjects, a subject in one set has beaten a subject in the other set at least once.
\\

Here we state an equivalent condition. Given the comparison comparison results $a_{ij}$, we can build a directed graph $G'$ whose adjacency matrix $A'$ satisfies $A'_{ij}=a_{ij}A_{ij}$.

\begin{theorem}
Condition A is equivalent with the strongly connectivity of $G'$.
\end{theorem}
\begin{proof}
Condition A says that for any partition $(V_1, V_2)$ of the vertices, there are at least one edge from $V_1$ to $V_2$ and also at least one edge from $V_2$ to $V_1$. If $G'$ is strongly connected, Condition A directly holds. Otherwise, the condensation of $G'$ has at least two points. We pick one strongly connected component with no indegree as $V_1$ and other vertices as $V_2$, then Condition A fails.
\end{proof}
\vbox{}

To approach our main consistency theorem, we first state that $G'$ is strongly connected with high probability for graphs with large spectral gaps and the merits with certain bounds.
For a $d$-regular expander $G(V,E)$, its expansion ratio is defined as
\[h(G)=\min_{0<|S|\leq n} \frac{|\partial S|}{|S|},\]
where $\partial S:=\{(u,v)\in E\mid u\in S,v\in V(G)\setminus S\}.$ Given the adjacency matrix $A$ and its spectrum $d=\lambda_1\geq \lambda_2\geq \cdots\geq \lambda_{n+1}$, \citet{alon2011eigenvalues} showed that $h(G)\geq \frac{1}{2}(d-\lambda_2)$, i.e., a large spectral gap guarantees a large expansion ratio. From now on, we will assume that a large spectral gap always exists, i.e., $\lambda_2\leq \frac{2}{d}$. There is lot of literature proving the existence of such expanders, even we restrict our attention to random biregular bipartite graphs which is the case in our application.

\begin{theorem}[\cite{brito2018spectral}]
Let $A$ be the adjacency matrix of a bipartite, biregular
random graph $G\sim\mathcal G(n, m, d_1, d_2)$. Without loss of generality, assume $d_1 \geq d_2$ or, equivalently, $n \leq m$. Then its second largest eigenvalue $\lambda_2(A)$ satisfies
\[\lambda_2(A)\leq \sqrt{d_1-1}+\sqrt{d_2-1}+\varepsilon_n'\] asymptotically almost surely, with $\varepsilon_n'\to 0$ as $n\to\infty$.
\end{theorem}

More specifically, we consider any instance $(G, \boldsymbol{u})$ that contains $n+1$ subjects where $G$ is a $d$-regular expander with adjacency matrix $A$ and its second largest eigenvalue satisfies $\lambda_{2}(A)\leq \frac{d}{2}$. Denote
\[\alpha=\max_{0\leq i,j\leq n}\frac{u_{i}}{u_{j}}\]
as the relative span of the merits.
\begin{theorem}
The directed comparison graph $G'$ with adjacency matrix $A'$ satisfies
\[\Pr\left[G'\text{is not strongly connected}\right]\leq 2\left(e^{(n+1)2^{-\frac{d}{4\alpha}}}-1\right).\]
\end{theorem}

\begin{proof}
For an edge between vertex $i$ and $j$ in $G$, i.e. $A_{ij}=1$, the corresponding directed edge in $G'$ goes from $i$ to $j$ with probability 
\[\Pr[A'_{ij}=1]=\Pr[a_{ij}=1]\leq \max_{0\leq i,j\leq n} \frac{u_i}{u_i+u_j}\leq \frac{\alpha}{1+\alpha}\leq 2^{-\frac{1}{\alpha}}.\]
Now consider any subset of vertices $S,1\leq |S|\leq \lfloor \frac{n+1}{2}\rfloor$, there are at least $h(G)|S|$ edges that connect $S$ and $V(G)\setminus S$ in $G$. The probability that all these edges go in the same direction in $G'$ is no more than
\[2^{1-\frac{h(G)|S|}{\alpha}}.\]
According to the equivalence, the probability that $G'$ is not strongly connected is no more than
\begin{equation*}
\begin{aligned}
    &\sum_{i=1}^{\lfloor \frac{n+1}{2}\rfloor}\binom{n+1}{i}2^{1-\frac{h(G)}{\alpha}i}\\
    \leq &  2\left(\sum_{i=0}^{n+1}\binom{n+1}{i}2^{-\frac{h(G) }{\alpha}i}-1\right)\\
    \leq & 2\left((1+2^{-\frac{h(G)}{\alpha}})^{n+1}-1\right)\\
    \leq & 2\left(e^{(n+1)2^{-\frac{h(G)}{\alpha}}}-1\right)\\
    \leq & 2\left(e^{(n+1)2^{-\frac{d}{4\alpha}}}-1\right)
\end{aligned}
\end{equation*}
\end{proof}

In the next step, we observe the likelihood equation \eqref{eq:likelihood:foc}. In the LHS, $a_i$ is the sum of $d$ independent Bernoulli variables whose expectation has the same format as the RHS except replacing $\boldsymbol{u^*}$ with $\boldsymbol{u}$. Formally,

\begin{theorem}
With probability $1-\delta-2\left(e^{(n+1)2^{-\frac{d}{4\alpha}}}-1\right)$, the MLEs exist and for any $0\leq i\leq n$,
\[\left|\sum_{j=0}^n\frac{A_{ij}u_i}{u_i+u_j}-\sum_{j=0}^n\frac{A_{ij}u^*_i}{u^*_i+u^*_j}\right|\leq \sqrt{\frac{k}{2}\ln\frac{2(n+1)}{\delta}}\]
\end{theorem}

\begin{proof}
Since $a_i=\sum_{j=0}^n A_{ij}a_{ij}$ is a sum of $d$ Bernoulli variables, by Hoeffding's Inequality,
\[\Pr\left[\left|a_i-\sum_{j=0}^n \frac{A_{ij}u_i}{u_i+u_j}\right|=\left|a_i-\E\left[a_i\right]\right|\geq \sqrt{\frac{k}{2}\ln\frac{2(n+1)}{\delta}}\right]\leq \frac{\delta}{n+1}.\]
By union bound on the probability of the non-existence of the MLEs and large deviation on any $a_i$, we finish the proof.
\end{proof}

\begin{theorem}

\end{theorem}

\begin{proof}
Let $\beta = \max_{0\leq i\leq n}\frac{u_i^*}{u_i}$ and $\gamma = \min_{0\leq i\leq n}\frac{u_i^*}{u_i}$.

For any $0\leq i\leq n$,
\begin{equation}
\begin{aligned}
    \left|\sum_{j=0}^n A_{ij}\left(\frac{u_i}{u_i+u_j}-\frac{u_i^*}{u_i^*+u_j^*}\right)\right|&=\left|\sum_{j=0}^nA_{ij}\frac{u_iu_j^*-u_i^*u_j}{(u_i+u_j)(u_i^*+u_j^*)}\right|=\left|\sum_{j=0}^nA_{ij}\frac{\frac{u_j^*}{u_j}-\frac{u_i^*}{u_i}}{(1+\frac{u_j}{u_i})(\frac{u_i^*}{u_i}\frac{u_i}{u_j}+\frac{u_j^*}{u_j})}\right|\\
    &\geq \left|\sum_{j=0}^nA_{ij}\frac{\frac{u_j^*}{u_j}-\frac{u_i^*}{u_i}}{\beta(1+\frac{u_j}{u_i})(1+\frac{u_i}{u_j}}\right|
\end{aligned}
\end{equation}
\end{proof}


\subsection{Setting}

There are $n$ students in class and $m$ questions in the question bank. We assume that the event of student $i$ correctly answering question $j$ can be described as a Bernoulli random variable $w_{ij}$, where $w_{ij}=1$ represents a correct answer and $w_{ij}=0$ represents a wrong answer.

The principal would like to measure the students' performance on the whole question bank. Thus an ideal grading rule for students would be their expected accuracy on a uniform question in the bank. \[\forall~i,\mathrm{opt}_i=\E_{j\sim \mathcal U([m])}[w_{ij}].\]

An exam $S$ can be described as a set of student-question pairs. After the exam, the principal observes the value of all $w_{ij}$s, where $(i,j)\in S$. Note that to avoid cheating, the principal would choose not to exhaust all possible pairs in one exam.

One traditional way to grade the student is averaging, i.e., use the ratio of the number of correct answers of the student to the total number of questions he received in the exam as his grade. \[\forall~i,\mathrm{avg}_i=\frac{\sum_{(i,j)\in S}w_{ij}}{\sum_{(i,j)\in S}1}.\]
It can be seen that if the exam is composed of uniformly random questions, the averaging is an unbiased estimator of the ideal grading rule.
\[\forall~i,\E_S[\mathrm{avg}_i]=\mathrm{opt}_i\]
However, we will show that, after the principal decides the exam, large bias occurs if we use averaging. An intuition is, some students are lucky and receive easier questions while some students are unlucky and receive harder questions.

